Qwen-MT-Lumen at WMT2026: Instruction-Specialized Translation via Quality-Aware Training and On-Policy Distillation

We present Lumen, The open-source model is available at, our submission to the WMT 2026 General Machine Translation Shared Task. We focus on instruction-specialized translation, where systems must produce accurate translations while satisfying fine-grained requirements on style, terminology, and structured output. Lumen follows a four-stage pipeline. First, continued pre-training and supervised fine-tuning jointly strengthen multilingual translation competence and the ability to follow translation-specific instructions, such as terminology, style, and format constraints. Second, we extend the originally offline M^{2}PO preference-optimization framework into an online preference-optimization stage: the current policy samples candidate translations, an LLM judge assigns continuous direct-assessment scores, and the resulting multi-pair preferences are used to update the model. Third, on-policy distillation transfers stronger translation-instruction-following behavior from a larger teacher model to the Qwen3-14B student, improving translation-instruction adherence while retaining a 14B primary translation backbone. Finally, structure-aware inference and postprocessing preserve required formats, while selective repair addresses clear structural or decoding failures before submission. We participate in 23 translation directions. Under an absolute 1--5 LLM-judge rubric that evaluates translation-instruction following and translation quality separately, Lumen reaches an overall mean score of 4.60. Despite using a 14B translation backbone, it achieves performance comparable to leading proprietary systems in both translation quality and translation-instruction following.

==> generated_report.tex <==
\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{Czech-Ukrainian}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 1.9 & 1.3 & 0.681 & \validated} \\
\opentrack{IKUN & 2.3 & 1.6 & 0.664 & \validated} \\
\opentrack{Aya23 & 2.5 & 1.9 & 0.665 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.6 & 2.0 & 0.661 & } \\
CUNI-Transformer & 3.0 & 2.0 & 0.639 & \validated \\
IKUN-C & 3.0 & 2.4 & 0.648 & \validated \\
\midrule
CycleL & 21.0 & 19.5 & 0.146 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for Czech-Ukrainian (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 0.9 & 0.719 & \validated} \\
\closedtrack{\nonsupporting{Claude-3.5} & 1.7 & 1.0 & 0.683 & \validated} \\
\opentrack{IOL-Research & 1.9 & 1.3 & 0.681 & \validated} \\
\closedtrack{\nonsupporting{CommandR-plus} & 1.9 & 1.3 & 0.677 & \validated} \\
\closedtrack{\nonsupporting{GPT-4} & 2.0 & 1.4 & 0.677 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 2.0 & 1.2 & 0.668 & \validated} \\
\closedtrack{ONLINE-W & 2.3 & 1.4 & 0.661 & \validated} \\
\closedtrack{\nonsupporting{Mistral-Large} & 2.3 & 1.6 & 0.666 & } \\
\opentrack{IKUN & 2.3 & 1.6 & 0.664 & \validated} \\
\opentrack{Aya23 & 2.5 & 1.9 & 0.665 & \validated} \\
\closedtrack{TranssionMT & 2.6 & 1.5 & 0.648 & } \\
\closedtrack{ONLINE-B & 2.6 & 1.6 & 0.648 & } \\
\closedtrack{ONLINE-A & 2.6 & 1.5 & 0.647 & } \\
\opentrack{\nonsupporting{Llama3-70B} & 2.6 & 2.0 & 0.661 & } \\
\closedtrack{ONLINE-G & 2.8 & 1.8 & 0.639 & } \\
CUNI-Transformer & 3.0 & 2.0 & 0.639 & \validated \\
IKUN-C & 3.0 & 2.4 & 0.648 & \validated \\
\midrule
\closedtrack{\nonsupporting{Phi-3-Medium} & 9.1 & 6.5 & 0.425 & } \\
\closedtrack{BJFU-LPT $\dagger$ & 11.5 & 7.6 & 0.321 & } \\
CycleL & 21.0 & 19.5 & 0.146 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for Czech-Ukrainian.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Czech}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
CUNI-MH & 2.1 & 2.3 & 0.690 & \validated \\
CUNI-GA & 2.3 & 3.7 & 0.726 & \validated \\
\opentrack{IOL-Research & 2.8 & 3.0 & 0.676 & \validated} \\
SCIR-MT & 3.2 & 3.3 & 0.664 & \validated \\
\opentrack{IKUN & 3.9 & 3.7 & 0.638 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 4.1 & 4.0 & 0.640 & \validated} \\
\opentrack{Aya23 & 4.3 & 4.0 & 0.630 & \validated} \\
CUNI-DocTransformer & 4.4 & 4.0 & 0.621 & \validated \\
IKUN-C & 4.7 & 4.3 & 0.618 & \validated \\
CUNI-Transformer $\dagger$ & 4.7 & 4.3 & 0.614 &  \\
\midrule
TSU-HITs & 19.5 & 16.6 & 0.235 &  \\
CycleL2 & 24.2 & 19.5 & 0.077 &  \\
CycleL & 27.0 & 22.5 & 0.031 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Czech (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 1.8 & 0.732 & \validated} \\
\closedtrack{\nonsupporting{Claude-3.5} & 2.1 & 2.4 & 0.693 & \validated} \\
CUNI-MH & 2.1 & 2.3 & 0.690 & \validated \\
CUNI-GA & 2.3 & 3.7 & 0.726 & \validated \\
\closedtrack{Gemini-1.5-Pro & 2.6 & 2.8 & 0.678 & \validated} \\
\closedtrack{\nonsupporting{GPT-4} & 2.6 & 2.9 & 0.682 & \validated} \\
\opentrack{IOL-Research & 2.8 & 3.0 & 0.676 & \validated} \\
\closedtrack{ONLINE-W & 2.8 & 2.8 & 0.669 & \validated} \\
\closedtrack{\nonsupporting{CommandR-plus} & 2.9 & 2.9 & 0.669 & \validated} \\
SCIR-MT & 3.2 & 3.3 & 0.664 & \validated \\
\closedtrack{TranssionMT & 3.5 & 3.5 & 0.655 & } \\
\closedtrack{ONLINE-A & 3.6 & 3.4 & 0.648 & } \\
\closedtrack{\nonsupporting{Mistral-Large} & 3.7 & 3.6 & 0.647 & } \\
\opentrack{IKUN & 3.9 & 3.7 & 0.638 & \validated} \\
\closedtrack{ONLINE-B & 4.0 & 3.9 & 0.640 & } \\
\opentrack{\nonsupporting{Llama3-70B} & 4.1 & 4.0 & 0.640 & \validated} \\
\opentrack{Aya23 & 4.3 & 4.0 & 0.630 & \validated} \\
CUNI-DocTransformer & 4.4 & 4.0 & 0.621 & \validated \\
IKUN-C & 4.7 & 4.3 & 0.618 & \validated \\
CUNI-Transformer $\dagger$ & 4.7 & 4.3 & 0.614 &  \\
\closedtrack{ONLINE-G & 5.7 & 5.2 & 0.592 & } \\
\midrule
\closedtrack{NVIDIA-NeMo $\dagger$ & 7.6 & 6.5 & 0.536 & } \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 15.0 & 11.4 & 0.305 & } \\
TSU-HITs & 19.5 & 16.6 & 0.235 &  \\
CycleL2 & 24.2 & 19.5 & 0.077 &  \\
CycleL & 27.0 & 22.5 & 0.031 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Czech.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-German}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 2.3 & 1.6 & 0.692 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.5 & 1.7 & 0.686 & \validated} \\
\opentrack{Aya23 & 2.7 & 1.8 & 0.680 & \validated} \\
\opentrack{IKUN & 3.0 & 1.8 & 0.668 & \validated} \\
IKUN-C & 3.8 & 2.0 & 0.641 & \validated \\
\opentrack{CUNI-NL & 4.2 & 2.1 & 0.624 & } \\
\midrule
AIST-AIRC & 7.2 & 3.3 & 0.551 &  \\
\opentrack{Occiglot & 8.2 & 3.8 & 0.539 & } \\
MSLC & 11.9 & 4.4 & 0.390 &  \\
TSU-HITs & 13.3 & 5.6 & 0.395 &  \\
CycleL2 & 27.0 & 11.5 & 0.091 &  \\
CycleL & 27.0 & 11.5 & 0.091 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-German (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 1.1 & 0.723 & \validated} \\
\closedtrack{Dubformer & 1.8 & 1.2 & 0.694 & \validated} \\
\closedtrack{TranssionMT & 1.8 & 1.4 & 0.699 & \validated} \\
\closedtrack{GPT-4 & 1.8 & 1.4 & 0.700 & \validated} \\
\closedtrack{ONLINE-B & 1.8 & 1.4 & 0.698 & \validated} \\
\closedtrack{Claude-3.5 & 1.9 & 1.4 & 0.695 & \validated} \\
\closedtrack{CommandR-plus & 2.0 & 1.4 & 0.696 & \validated} \\
\closedtrack{Mistral-Large & 2.0 & 1.5 & 0.694 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 2.2 & 1.5 & 0.688 & \validated} \\
\closedtrack{ONLINE-W & 2.2 & 1.5 & 0.689 & } \\
\opentrack{IOL-Research & 2.3 & 1.6 & 0.692 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.5 & 1.7 & 0.686 & \validated} \\
\opentrack{Aya23 & 2.7 & 1.8 & 0.680 & \validated} \\
\opentrack{IKUN & 3.0 & 1.8 & 0.668 & \validated} \\
\closedtrack{ONLINE-A & 3.0 & 1.8 & 0.667 & } \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 3.4 & 2.0 & 0.657 & } \\
\closedtrack{ONLINE-G & 3.5 & 2.1 & 0.662 & } \\
IKUN-C & 3.8 & 2.0 & 0.641 & \validated \\
\opentrack{CUNI-NL & 4.2 & 2.1 & 0.624 & } \\
\midrule
AIST-AIRC & 7.2 & 3.3 & 0.551 &  \\
\closedtrack{NVIDIA-NeMo $\dagger$ & 7.4 & 3.5 & 0.558 & } \\
\opentrack{Occiglot & 8.2 & 3.8 & 0.539 & } \\
MSLC & 11.9 & 4.4 & 0.390 &  \\
TSU-HITs & 13.3 & 5.6 & 0.395 &  \\
CycleL2 & 27.0 & 11.5 & 0.091 &  \\
CycleL & 27.0 & 11.5 & 0.091 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-German.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Spanish}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 2.3 & 2.8 & 0.701 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.6 & 3.0 & 0.693 & \validated} \\
\opentrack{IKUN & 2.8 & 3.3 & 0.687 & \validated} \\
\opentrack{Aya23 & 3.1 & 3.5 & 0.681 & } \\
IKUN-C & 3.4 & 3.5 & 0.666 & \validated \\
\opentrack{Occiglot & 5.9 & 5.4 & 0.583 & } \\
MSLC & 7.4 & 6.4 & 0.532 & \validated \\
\midrule
TSU-HITs & 16.3 & 14.2 & 0.289 &  \\
CycleL & 24.0 & 20.9 & 0.072 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Spanish (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 1.9 & 0.745 & \validated} \\
\closedtrack{GPT-4 & 1.9 & 2.5 & 0.712 & \validated} \\
\closedtrack{Dubformer & 2.0 & 2.2 & 0.700 & \validated} \\
\closedtrack{CommandR-plus & 2.1 & 2.6 & 0.706 & \validated} \\
\closedtrack{Claude-3.5 & 2.1 & 2.6 & 0.705 & \validated} \\
\closedtrack{Mistral-Large & 2.2 & 2.7 & 0.707 & \validated} \\
\opentrack{IOL-Research & 2.3 & 2.8 & 0.701 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 2.4 & 2.8 & 0.696 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.6 & 3.0 & 0.693 & \validated} \\
\closedtrack{ONLINE-B $\dagger$ & 2.7 & 3.1 & 0.690 & \validated} \\
\closedtrack{ONLINE-W & 2.7 & 3.0 & 0.682 & } \\
\closedtrack{TranssionMT & 2.8 & 3.2 & 0.689 & } \\
\opentrack{IKUN & 2.8 & 3.3 & 0.687 & \validated} \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 3.0 & 3.4 & 0.685 & } \\
\closedtrack{ONLINE-A & 3.0 & 3.3 & 0.676 & } \\
\opentrack{Aya23 & 3.1 & 3.5 & 0.681 & } \\
\closedtrack{ONLINE-G & 3.2 & 3.6 & 0.674 & } \\
IKUN-C & 3.4 & 3.5 & 0.666 & \validated \\
\closedtrack{NVIDIA-NeMo $\dagger$ & 4.5 & 4.4 & 0.631 & } \\
\opentrack{Occiglot & 5.9 & 5.4 & 0.583 & } \\
MSLC & 7.4 & 6.4 & 0.532 & \validated \\
\midrule
TSU-HITs & 16.3 & 14.2 & 0.289 &  \\
CycleL & 24.0 & 20.9 & 0.072 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Spanish.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Hindi}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 2.1 & 4.3 & 0.622 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.1 & 4.6 & 0.630 & \validated} \\
\opentrack{Aya23 & 3.2 & 5.4 & 0.591 & \validated} \\
IKUN-C & 5.5 & 7.1 & 0.499 & \validated \\
\midrule
\opentrack{IKUN & 7.7 & 9.4 & 0.428 & } \\
CycleL & 20.0 & 23.4 & 0.083 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Hindi (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 3.1 & 0.657 & \validated} \\
\closedtrack{\nonsupporting{Claude-3.5} & 1.2 & 3.3 & 0.649 & \validated} \\
\closedtrack{TranssionMT & 1.3 & 3.3 & 0.644 & \validated} \\
\closedtrack{ONLINE-B & 1.4 & 3.3 & 0.641 & \validated} \\
\closedtrack{\nonsupporting{Gemini-1.5-Pro} & 1.6 & 3.6 & 0.635 & \validated} \\
\closedtrack{\nonsupporting{GPT-4} & 2.1 & 4.5 & 0.628 & \validated} \\
\opentrack{IOL-Research & 2.1 & 4.3 & 0.622 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.1 & 4.6 & 0.630 & \validated} \\
\closedtrack{\nonsupporting{CommandR-plus} & 2.3 & 4.4 & 0.612 & } \\
\opentrack{Aya23 & 3.2 & 5.4 & 0.591 & \validated} \\
\closedtrack{ONLINE-A & 3.5 & 6.2 & 0.590 & } \\
\closedtrack{ONLINE-G & 4.2 & 7.4 & 0.583 & } \\
\closedtrack{\nonsupporting{Mistral-Large} & 5.0 & 7.7 & 0.541 & } \\
IKUN-C & 5.5 & 7.1 & 0.499 & \validated \\
\closedtrack{NVIDIA-NeMo $\dagger$ & 5.8 & 8.9 & 0.530 & } \\
\midrule
\closedtrack{\nonsupporting{Phi-3-Medium} & 7.4 & 10.7 & 0.483 & } \\
\opentrack{IKUN & 7.7 & 9.4 & 0.428 & } \\
\closedtrack{ONLINE-empty & 15.3 & 20.9 & 0.296 & } \\
CycleL & 20.0 & 23.4 & 0.083 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Hindi.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Icelandic}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IKUN & 3.2 & 4.3 & 0.666 & \validated} \\
\opentrack{AMI & 3.7 & 4.9 & 0.663 & \validated} \\
IKUN-C & 3.7 & 4.9 & 0.657 & \validated \\
\opentrack{IOL-Research & 4.3 & 5.7 & 0.655 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 6.7 & 8.0 & 0.586 & \validated} \\
\midrule
\opentrack{\nonsupporting{Aya23} & 15.2 & 14.9 & 0.311 & } \\
TSU-HITs & 19.2 & 18.4 & 0.192 &  \\
CycleL & 21.0 & 20.2 & 0.148 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Icelandic (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 2.5 & 0.740 & \validated} \\
\closedtrack{\nonsupporting{Claude-3.5} & 2.3 & 3.6 & 0.697 & \validated} \\
\closedtrack{Dubformer & 2.5 & 3.4 & 0.685 & \validated} \\
\opentrack{IKUN & 3.2 & 4.3 & 0.666 & \validated} \\
\closedtrack{GPT-4 & 3.4 & 4.7 & 0.673 & \validated} \\
\opentrack{AMI & 3.7 & 4.9 & 0.663 & \validated} \\
IKUN-C & 3.7 & 4.9 & 0.657 & \validated \\
\closedtrack{TranssionMT & 4.2 & 5.5 & 0.653 & } \\
\closedtrack{ONLINE-B $\dagger$ & 4.2 & 5.5 & 0.652 & \validated} \\
\opentrack{IOL-Research & 4.3 & 5.7 & 0.655 & \validated} \\
\closedtrack{ONLINE-A & 5.5 & 6.4 & 0.603 & } \\
\opentrack{\nonsupporting{Llama3-70B} & 6.7 & 8.0 & 0.586 & \validated} \\
\closedtrack{ONLINE-G & 6.9 & 7.9 & 0.573 & } \\
\midrule
\closedtrack{\nonsupporting{CommandR-plus} & 9.8 & 10.6 & 0.487 & } \\
\closedtrack{\nonsupporting{Mistral-Large} & 10.4 & 10.9 & 0.465 & } \\
\opentrack{\nonsupporting{Aya23} & 15.2 & 14.9 & 0.311 & } \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 16.2 & 15.7 & 0.278 & } \\
\closedtrack{ONLINE-empty & 18.1 & 19.5 & 0.296 & } \\
TSU-HITs & 19.2 & 18.4 & 0.192 &  \\
CycleL & 21.0 & 20.2 & 0.148 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Icelandic.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Japanese}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
Team-J & 1.9 & 2.9 & 0.740 & \validated \\
NTTSU & 1.9 & 2.6 & 0.731 & \validated \\
\opentrack{IOL-Research & 2.3 & 3.1 & 0.724 & \validated} \\
\opentrack{Aya23 & 2.3 & 3.1 & 0.719 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.6 & 3.5 & 0.714 & \validated} \\
\opentrack{IKUN & 3.1 & 3.7 & 0.696 & } \\
IKUN-C & 3.9 & 4.3 & 0.669 & \validated \\
\midrule
AIST-AIRC & 6.6 & 6.5 & 0.583 &  \\
UvA-MT & 6.7 & 6.7 & 0.589 &  \\
CycleL & 24.0 & 22.4 & 0.101 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Japanese (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 2.0 & 0.762 & \validated} \\
\closedtrack{ONLINE-B & 1.4 & 2.4 & 0.750 & \validated} \\
\closedtrack{Claude-3.5 & 1.5 & 2.3 & 0.744 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 1.7 & 2.5 & 0.734 & \validated} \\
\closedtrack{GPT-4 & 1.7 & 2.7 & 0.740 & \validated} \\
Team-J & 1.9 & 2.9 & 0.740 & \validated \\
NTTSU & 1.9 & 2.6 & 0.731 & \validated \\
\closedtrack{CommandR-plus & 1.9 & 2.7 & 0.730 & \validated} \\
\opentrack{IOL-Research & 2.3 & 3.1 & 0.724 & \validated} \\
\opentrack{Aya23 & 2.3 & 3.1 & 0.719 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 2.6 & 3.5 & 0.714 & \validated} \\
\closedtrack{DLUT-GTCOM & 2.6 & 3.0 & 0.697 & } \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 2.8 & 3.6 & 0.709 & } \\
\closedtrack{ONLINE-W & 2.9 & 3.6 & 0.700 & } \\
\closedtrack{\nonsupporting{Mistral-Large} & 2.9 & 3.8 & 0.707 & } \\
\closedtrack{ONLINE-A & 3.0 & 3.6 & 0.699 & } \\
\opentrack{IKUN & 3.1 & 3.7 & 0.696 & } \\
IKUN-C & 3.9 & 4.3 & 0.669 & \validated \\
\midrule
\closedtrack{ONLINE-G & 6.4 & 6.6 & 0.599 & } \\
AIST-AIRC & 6.6 & 6.5 & 0.583 &  \\
UvA-MT & 6.7 & 6.7 & 0.589 &  \\
\closedtrack{NVIDIA-NeMo $\dagger$ & 6.9 & 6.9 & 0.582 & } \\
CycleL & 24.0 & 22.4 & 0.101 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Japanese.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Russian}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 2.6 & 3.7 & 0.694 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 3.1 & 4.1 & 0.681 & \validated} \\
\opentrack{IKUN & 3.2 & 4.1 & 0.675 & \validated} \\
\opentrack{Aya23 & 3.3 & 4.2 & 0.669 & \validated} \\
IKUN-C & 3.9 & 4.7 & 0.649 & \validated \\
\midrule
CUNI-DS & 5.9 & 6.2 & 0.584 &  \\
TSU-HITs & 10.8 & 9.8 & 0.421 &  \\
CycleL & 24.3 & 22.2 & 0.062 &  \\
CycleL2 & 25.0 & 22.4 & 0.027 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Russian (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 2.4 & 0.742 & \validated} \\
\closedtrack{Dubformer & 1.9 & 2.8 & 0.701 & \validated} \\
\closedtrack{Yandex & 1.9 & 2.9 & 0.705 & \validated} \\
\closedtrack{Claude-3.5 & 2.0 & 3.0 & 0.706 & \validated} \\
\closedtrack{ONLINE-G & 2.2 & 3.3 & 0.706 & \validated} \\
\closedtrack{GPT-4 & 2.3 & 3.4 & 0.703 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 2.3 & 3.2 & 0.697 & \validated} \\
\closedtrack{\nonsupporting{CommandR-plus} & 2.4 & 3.4 & 0.693 & \validated} \\
\closedtrack{ONLINE-W & 2.6 & 3.5 & 0.688 & } \\
\opentrack{IOL-Research & 2.6 & 3.7 & 0.694 & \validated} \\
\closedtrack{\nonsupporting{Mistral-Large} & 2.7 & 3.7 & 0.692 & } \\
\opentrack{\nonsupporting{Llama3-70B} & 3.1 & 4.1 & 0.681 & \validated} \\
\closedtrack{ONLINE-B & 3.1 & 3.9 & 0.673 & } \\
\closedtrack{TranssionMT & 3.1 & 3.9 & 0.673 & } \\
\opentrack{IKUN & 3.2 & 4.1 & 0.675 & \validated} \\
\opentrack{Aya23 & 3.3 & 4.2 & 0.669 & \validated} \\
\closedtrack{ONLINE-A & 3.4 & 4.1 & 0.663 & } \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 3.9 & 4.7 & 0.654 & } \\
IKUN-C & 3.9 & 4.7 & 0.649 & \validated \\
\midrule
CUNI-DS & 5.9 & 6.2 & 0.584 &  \\
\closedtrack{NVIDIA-NeMo $\dagger$ & 7.2 & 7.3 & 0.549 & } \\
TSU-HITs & 10.8 & 9.8 & 0.421 &  \\
CycleL & 24.3 & 22.2 & 0.062 &  \\
CycleL2 & 25.0 & 22.4 & 0.027 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Russian.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Ukrainian}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 2.4 & 3.4 & 0.675 & \validated} \\
\opentrack{IKUN & 2.8 & 3.7 & 0.661 & \validated} \\
\opentrack{\nonsupporting{Llama3-70B} & 3.2 & 4.2 & 0.647 & } \\
\opentrack{Aya23 & 3.3 & 4.2 & 0.642 & } \\
IKUN-C & 3.9 & 4.7 & 0.622 & \validated \\
\midrule
CycleL & 21.0 & 22.4 & 0.037 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Ukrainian (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 2.2 & 0.732 & \validated} \\
\closedtrack{Dubformer & 1.8 & 2.7 & 0.691 & \validated} \\
\closedtrack{Claude-3.5 & 2.0 & 3.0 & 0.693 & \validated} \\
\closedtrack{ONLINE-W & 2.1 & 2.8 & 0.679 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 2.2 & 3.0 & 0.677 & \validated} \\
\closedtrack{\nonsupporting{CommandR-plus} & 2.3 & 3.2 & 0.678 & \validated} \\
\closedtrack{GPT-4 & 2.3 & 3.3 & 0.682 & \validated} \\
\closedtrack{ONLINE-G & 2.3 & 3.1 & 0.670 & } \\
\opentrack{IOL-Research & 2.4 & 3.4 & 0.675 & \validated} \\
\closedtrack{\nonsupporting{Mistral-Large} & 2.4 & 3.4 & 0.675 & } \\
\opentrack{IKUN & 2.8 & 3.7 & 0.661 & \validated} \\
\closedtrack{ONLINE-B & 3.1 & 3.9 & 0.646 & } \\
\closedtrack{TranssionMT & 3.1 & 4.0 & 0.646 & } \\
\opentrack{\nonsupporting{Llama3-70B} & 3.2 & 4.2 & 0.647 & } \\
\opentrack{Aya23 & 3.3 & 4.2 & 0.642 & } \\
\closedtrack{ONLINE-A & 3.3 & 4.1 & 0.634 & } \\
IKUN-C & 3.9 & 4.7 & 0.622 & \validated \\
\midrule
\closedtrack{NVIDIA-NeMo $\dagger$ & 6.2 & 7.0 & 0.537 & } \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 11.1 & 11.3 & 0.339 & } \\
CycleL & 21.0 & 22.4 & 0.037 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Ukrainian.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{English-Chinese}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 1.8 & 3.1 & 0.700 & \validated} \\
HW-TSC & 2.3 & 3.4 & 0.675 & \validated \\
\opentrack{\nonsupporting{Llama3-70B} & 2.8 & 3.9 & 0.662 & \validated} \\
\opentrack{Aya23 & 3.0 & 4.1 & 0.655 & \validated} \\
\opentrack{IKUN & 3.1 & 4.0 & 0.646 & \validated} \\
IKUN-C & 3.5 & 4.2 & 0.624 & \validated \\
UvA-MT $\dagger$ & 4.3 & 5.2 & 0.607 &  \\
\midrule
CycleL & 20.1 & 20.1 & 0.086 &  \\
CycleL2 & 22.0 & 22.1 & 0.030 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Chinese (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 2.3 & 0.726 & \validated} \\
\closedtrack{Claude-3.5 & 1.7 & 3.0 & 0.703 & \validated} \\
\closedtrack{ONLINE-B & 1.7 & 2.9 & 0.697 & \validated} \\
\opentrack{IOL-Research & 1.8 & 3.1 & 0.700 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 1.8 & 3.1 & 0.698 & \validated} \\
\closedtrack{GPT-4 & 2.0 & 3.3 & 0.693 & \validated} \\
\closedtrack{CommandR-plus & 2.2 & 3.3 & 0.681 & \validated} \\
\closedtrack{ONLINE-W & 2.2 & 3.2 & 0.677 & } \\
HW-TSC & 2.3 & 3.4 & 0.675 & \validated \\
\closedtrack{\nonsupporting{Mistral-Large} & 2.8 & 4.0 & 0.665 & } \\
\opentrack{\nonsupporting{Llama3-70B} & 2.8 & 3.9 & 0.662 & \validated} \\
\opentrack{Aya23 & 3.0 & 4.1 & 0.655 & \validated} \\
\opentrack{IKUN & 3.1 & 4.0 & 0.646 & \validated} \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 3.1 & 4.2 & 0.648 & } \\
\closedtrack{ONLINE-A & 3.3 & 4.1 & 0.636 & } \\
IKUN-C & 3.5 & 4.2 & 0.624 & \validated \\
UvA-MT $\dagger$ & 4.3 & 5.2 & 0.607 &  \\
\closedtrack{ONLINE-G & 4.8 & 5.5 & 0.588 & } \\
\midrule
\closedtrack{NVIDIA-NeMo $\dagger$ & 7.3 & 7.6 & 0.494 & } \\
CycleL & 20.1 & 20.1 & 0.086 &  \\
CycleL2 & 22.0 & 22.1 & 0.030 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for English-Chinese.}
\end{table*}


\clearpage
\begin{table*}
\centering
\begin{tabular}{c}
\bf{\Large{Japanese-Chinese}}
\vspace{1em}
\end{tabular}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\opentrack{IOL-Research & 2.2 & 3.9 & 0.593 & \validated} \\
Team-J & 2.8 & 4.0 & 0.570 & \validated \\
\opentrack{\nonsupporting{Llama3-70B} & 3.1 & 4.7 & 0.578 & \validated} \\
\opentrack{Aya23 & 3.7 & 5.0 & 0.563 & \validated} \\
\opentrack{NTTSU & 3.7 & 5.3 & 0.566 & \validated} \\
\opentrack{IKUN & 4.4 & 5.4 & 0.544 & \validated} \\
UvA-MT $\dagger$ & 5.2 & 6.3 & 0.534 &  \\
IKUN-C & 5.5 & 6.2 & 0.519 & \validated \\
\midrule
MSLC & 8.9 & 8.8 & 0.450 &  \\
CycleL & 23.0 & 21.5 & 0.202 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for Japanese-Chinese (excluding closed systems).}
\vspace{2em}
\begin{tabular}{R{40mm}C{22mm}C{19mm}C{22mm}C{32mm}}
\bf System Name & \bf AutoRank $\downarrow$ & \bf MetricX $\downarrow$ & \bf CometKiwi $\uparrow$ & \bf Human evaluation? \\
\toprule
\closedtrack{Unbabel-Tower70B & 1.0 & 3.2 & 0.622 & \validated} \\
\closedtrack{Claude-3.5 & 1.7 & 3.5 & 0.603 & \validated} \\
\closedtrack{Gemini-1.5-Pro & 1.9 & 3.5 & 0.595 & \validated} \\
\closedtrack{DLUT-GTCOM & 2.0 & 3.3 & 0.586 & \validated} \\
\closedtrack{GPT-4 & 2.1 & 3.8 & 0.597 & \validated} \\
\opentrack{IOL-Research & 2.2 & 3.9 & 0.593 & \validated} \\
\closedtrack{CommandR-plus & 2.8 & 4.1 & 0.576 & \validated} \\
Team-J & 2.8 & 4.0 & 0.570 & \validated \\
\opentrack{\nonsupporting{Llama3-70B} & 3.1 & 4.7 & 0.578 & \validated} \\
\closedtrack{\nonsupporting{Mistral-Large} & 3.5 & 4.9 & 0.568 & } \\
\opentrack{Aya23 & 3.7 & 5.0 & 0.563 & \validated} \\
\opentrack{NTTSU & 3.7 & 5.3 & 0.566 & \validated} \\
\closedtrack{\nonsupporting{Phi-3-Medium} & 4.0 & 5.1 & 0.552 & } \\
\opentrack{IKUN & 4.4 & 5.4 & 0.544 & \validated} \\
\closedtrack{ONLINE-B $\dagger$ & 5.2 & 5.5 & 0.518 & \validated} \\
UvA-MT $\dagger$ & 5.2 & 6.3 & 0.534 &  \\
\closedtrack{ONLINE-W & 5.3 & 6.0 & 0.522 & } \\
IKUN-C & 5.5 & 6.2 & 0.519 & \validated \\
\closedtrack{ONLINE-A & 6.8 & 6.8 & 0.484 & } \\
\midrule
MSLC & 8.9 & 8.8 & 0.450 &  \\
\closedtrack{ONLINE-G & 10.3 & 9.6 & 0.413 & } \\
CycleL & 23.0 & 21.5 & 0.202 &  \\
\bottomrule
\end{tabular}
\caption{Preliminary WMT24 General MT automatic ranking for Japanese-Chinese.}
\end{table*}
